Ontology Focusing: Knowledge-enriched Databases on Demand

We propose a novel framework to facilitate the on-demand design of data-centric systems by exploiting domain knowledge from an existing ontology. Its key ingredient is a process that we call focusing, which allows to obtain a schema for a (possibly knowledge-enriched) database semi-automatically, given an ontology and a specification of the scope of the desired system. We formalize the inputs and outputs of focusing, and identify relevant computational problems: finding a schema via focusing, testing its consistency, and answering queries in the knowledge-enriched databases it produces. These definitions are fully independent of the ontology language. We then instantiate the framework using selected description logics as ontology languages, and popular classes of queries for specifying the scope of the system. For several representative combinations, we study the decidability and complexity of the identified computational problems. As a by-product, we isolate (and solve) variants of classical decision problems in description logics, that are interesting in their own right.

==> 4-process.tex <==
\section{Process: Introduction}

In recent years, general purpose ontologies like WordNet
\cite{fellbaum98wordnet}, Yago \cite{SuchanekKW07}, or Schema.org
\cite{Patel-Schneider} are becoming increasingly rich and accurate. An
unavoidable cost to pay is that they are getting larger and
larger. Suppose a  wants to design a specialized system based
on one of such ontologies. They face two---potentially
conflicting---challenges. On one hand, only the part of the ontology
that is relevant should be incorporated into the system, to avoid
unnecessary slow-down. On the other hand, the ontology itself may not
be suffcient: the system may need that certain predicates (say, issued
invoices or performed surgeries) be manually maintained in a database,
rather than relying on the general knowledge about them represented in
the ontology. Thus, the goal of the developer is to extract a smaller
ontology and a database that would together constitute a knowledge
base around which the specialized system would be built. To what
extent can this be automatized? In what follows we isolate a
collection of tasks that need to be solved in the process.




\section{Framework}


The starting point is an ontology $\Oo$. At the current stage we shall
think about it as a theory expressed in some logical formalism, over a
relational signature $\Sigma$ with constants. We shall be working with
the unique name assumption, assuming that all constants are elements
of the domain of each structure over $\Sigma$, and are always
interpreted as themselves. A fundamental assumption we make is that
the designer trusts the ontology. That is, their design decisions only
restrict the class of possible models, but never revoke knowledge by
allowing more models.

Based on some specification of the scope, the designer needs to chose
the predicates to be maintained in the database, and the predicates to
be eliminated. Let us focus on the first issue.


\subsection{Schema extraction}

What exactly does it mean that a predicate is maintained? There are
two decisions to be made about each predicate: whether it will evolve
during the run of the system, and whether it should be viewed as an
accurate representation of reality or just an under-approximation.
%
The first choice splits the predicates in to \emph{static} and
\emph{dynamic} ones. The static ones are only represented in the
ontology, while the dynamic ones are kept in the database and can be
updated as the system runs.
%
The second choice splits the dynamic predicates into \emph{closed} and
\emph{open} ones. If a dynamic predicate is closed, we only allow
interpretations that agree with the current contents of this predicate
in the database. For open dynamic predicates, we allow all supersets
of the current contents of this predicate.
%
This gives three kinds of predicates.

\begin{description}
\item[Closed dynamic predicates] represent aspects of reality fully
  observable---and often fully controlled---by the system, 
  like money transfers in a banking platform. A predicate should be
  closed dynamic if it is crucial for the system.
\item[Open dynamic predicates] represent aspects of reality that are
  only partially observed by the system, like customer preferences
  following from their behaviour. A predicate should be open dynamic
  if its contents is helpful, but its completeness is not required.
\item[Static predicates] correspond to aspects of reality for which
  the system will fully rely on the ontology. These may include
  absolute truths, like the seven days of the week, unobservable
  facts, like the dream car of a customer, and irrrelevant
  information, like the phase of the moon.  A predicate should be
  static, if the knowledge about it stored in the ontology is
  sufficient from the point of view of the scope of the system under design. 
\end{description}
%
% Static predicates describe
% aspects of reality that do not change and are completely represented
% in the ontology, like the seven days of the week. Open static
% predicates correspond to aspects of reality about which the ontology
% has only partial information; the information is not updated by the
% system, possibly because these aspects cannot or need not be observed,
% like the phase of the moon.
%

% Intuitively, a predicate should be closed
% dynamic if it is crucial for the system, and the system must fully
% maintain it. A predicate should be open dynamic if its content is
% helpful, but it cannot be fully maintained. It should be open static,
% if there is no way or no need to update the predicate. It should be
% closed static if we believe that the knowledge about this predicate
% originally represented in the ontology can be considered complete in
% the restricted fragment of reality in the scope of the system. 

%%% In fact, we should also allow static closed predicates with chosen
%%% content, but this would make the picture to complicated. This can
%%% be done beforehand, by manually extending the ontology. We should
%%% explain as well that one can add some domain knowledge to the
%%% general ontology.


The partition of $\Sigma$ into the three categories clearly depends on
the scope of the system. How does one specify the scope? Intuitively,
we need to maintain a predicate if its contents might need to be
returned at some point. Suppose that we know in advance all queries to
be posed when the system is functioning. Because queries posed to the
system's database typically use constants input by users, it may seem
unrealistic. But these constants can be easily abstracted away by
replacing them with free variables (to be returned).
%%% This should be turned into a lemma. First just go with some
%%% queries, and then say that if we replace them with queries
%%% hardcoded into the system, with constants treated as variables, we
%%% get completeness of the specialised queries as well. 
Now, when is a set of maintained predicates sufficient to support
these queries? The reason we need a record in a database is that we
want to guarantee completeness of the returned answers.

% that it is returned regardless of the 
% possible reasoning going on in the background. That is, we would like
% the answers to these queries to depend exclusively on the content of
% the maintained predicates. The intended meaning is that for each
% interpretation of the maintained predicates, the answers to these
% queries do not depend on the interpretation of the unmaintained
% predicates (as long as the whole structure satisfies the ontology).

What does it mean that query $Q$ returns a complete answer? Speaking
of completeness only makes sense if we assume the existence of a model
$\Mm$ that our KB instance incompletely represents. Recall that the KB
consists of a database instance $\Dd$ over the dynamic predicates and
an ontology $\Oo$, such that $\Mm \models \Dd, \Oo$. The KB $(\Dd,
\Oo)$ is \emph{complete} for query $Q$ with respect to $\Mm$ if for
all tuples $\bar a$,
\[\Dd, \Oo \models Q(\bar a) \iff \Mm \models Q(\bar a)\,.\]
But we are not interested in a specific KB, but in all KBs possible
for the chosen partition of $\Sigma$ into closed dynamic predicates
$\Sigma_c$, and open dynamic predicates $\Sigma_o$, and static
predicates $\Sigma_s$. We would like to guarantee that for each $\Mm$,
each representation $(\Dd, \Oo)$ of $\Mm$ is complete for $Q$
wrt. $\Mm$, or equivalently, if for each $\Dd$  over $\Sigma_c\cup
\Sigma_o$, the KB $(\Dd, \Oo)$ is complete for $Q$ with respect to
each model $\Mm$ of $(\Dd, \Oo)$. 

We shall say that $\Sigma_0 \subseteq \Sigma$ \emph{supports} $Q$ if
for each $\Dd$ over $\Sigma_c$, the KB $(\Dd, \Oo)$ is complete for $Q$
with respect to each model $\Mm$ of $\Oo$ that agrees with $\Dd$.
%
% that is, for each $\Mm$, for each $\Dd$ over $\Sigma_c\cup \Sigma_o$,
% \[\Mm \models \Dd, \Oo \implies (\Dd,\Oo) \text{ is complete for } Q
% \text{ wrt } \Mm \,.\]
The following lemma offers a straightforward but
informative equivalent characterisation. 

\begin{lemma} \label{lem:support}
  $\Sigma_0 \subseteq \Sigma$ supports $Q$ iff
  for each $\bar a$ and each $\Dd$ over $\Sigma_0$, 
  \[\Mm \models Q(\bar a) \iff \Mm' \models Q(\bar a)\]
  for all models $\Mm$ and $\Mm'$ of $\Oo$
  that agree with $\Dd$.
\end{lemma}

That is, either each model $\Mm$ of $\Oo$ agreeing with $\Dd$
satisfies $Q(\bar a)$ or none does. Intuitively, this means that each
$\Dd$ over $\Sigma_0$ contains all the information relevant for $Q$
(in the presence of the ontology $\Oo$). This intuiton is reinforced
by the following lemma.

\begin{lemma} \label{lem:support-complete}
For each partition of $\Sigma$ into $\Sigma_c$, $\Sigma_o$, and
$\Sigma_s$, it holds that $\Sigma_c$ supports $Q$ iff for each model
$\Mm$, each representation of $\Mm$ is complete for $Q$ with respect
to $\Mm$. 
\end{lemma}

\begin{proof}
The claim follows from Lemma~\ref{lem:support}. 
\end{proof}

Lemma~\ref{lem:support-complete} tells us that from the point of view
of completeness, it suffices to ensure that the chosen set of closed
dynamic predicates supports all specified queries. It is clear
that this condition is monotone: if some set supports $Q$, so
will all its supersets. Efficiency suggest taking a minimal set
supporting all specified queries, possibly applying some heuristics to
chose between multiple minimal candidates, in order to further
optimize the size of the stored predicates.  But how do we test if a
given set of predicates supports a given query? 

%
% \begin{remark}
% If the logic used to express ontologies is strong enough, we can
% eliminate open dynamic predicates by declaring them static and
% introducing a closed dynamic predicate contained in them. 
% \end{remark}
%

\begin{lemma} \label{lem:support-reduction}
Let $\Sigma_0 \subseteq \Sigma$. Let $\Oo'$ and $Q'$ be obtained from
$\Oo$ and $Q$, respectively, by replacing each predicate $P\in\Sigma -
\Sigma_0$ by its fresh copy $P'$. Then, $\Sigma_0$ supports $Q$ under $\Oo$
iff $Q \subseteq Q'$ over all models of $\Oo \cup \Oo'$ with finite
interpretations of predicates from $\Sigma_0$.
\end{lemma}

\begin{proof}
Also follows from Lemma~\ref{lem:support}. 
\end{proof}

Lemma~\ref{lem:support-reduction} reduces testing support to query
containment modulo ontology, over models where some predicates are
required to be finite; the remaining predicates are either finite as
well, or unrestricted, depending on the chosen mode of reasoning. 
%
By including the first query into the ontology (for conjunctive
queries this is possible in virtually all ontology formalisms), we further
reduce the problem to ontology mediated query answering (OMQA), again with
the additional condition that interpretations of certain predicates
are finite. When we reason in the finite mode, or when our logic has
finite controllability, the additional consition trivialises, and we
end up with the usual OMQ. But if we reason in the unrestricted mode
and our logic does not have finite controllability, this is an
entirely new problem, different from the unrestricted OMQA and the
finite OMQA.


% For this task there is hardly any prior work. The natural starting
% points are the logics ALCIF and S. For ALCIF, decidability both for
% the unrestricted and finite case is obtained by reduction to the
% satisfiability of the two-variable guarded fragment of first order
% logic with counting \cite{Pratt-Hartmann09}. The algorithms for this
% problem in the finite and the unrestricted case
% \cite{Pratt-Hartmann07}, seem to be compatible enough to give solution
% for the mixed case. Whether this carries over to ALCIF, requires a
% careful examination of the reduction, non-trivial itself. For S,
% initial research shows that the algorithms for the two cases are not
% directly compatible, and despite the simplicity of this logic, some
% new ideas are needed.

% We can see from Lemma~\ref{lem:support} that what actually matters for
% completeness is $\Sigma_c\cap\Sigma_d$ and $\Sigma_c\cap
% \Sigma_s$. It is also intutively clear, that the larger $\Sigma_c\cap
% \Sigma_s$, the smaller $\Sigma_c\cap\Sigma_d$ may need to be, as
% there is less potential offending instances. So, there seems to be a
% certain trade-off here. We propose to proceed as follows. For 
% $\Sigma_c\cap \Sigma_s$ take the set of closed predicates from the
% ontology. Then, if some $\Sigma_c\cap\Sigma_d$ supports $Q$, it will
% also support $Q$ if we make $\Sigma_c\cap \Sigma_s$ greater. (If some
% closed dynamic predicates are assumed to be static, that is fine as
% well.) Then, a natural choice is to take a minimal
% $\Sigma_c\cap\Sigma_d$ that supports $Q$.


\subsection{Module extraction}
 
Given $\Sigma_c^0$, $\Sigma_m^0$, $\Sigma_f^0$, $\Sigma_\bot^0$,
partition  $\Sigma$ into $\Sigma_c$, $\Sigma_m$, $\Sigma_s$, $\Sigma_\bot$, such that
\[\Sigma_c^0 \subseteq \Sigma_c,\quad \Sigma_m^0 \subseteq \Sigma_s \cup
\Sigma_m,\quad \Sigma_s^0 \subseteq \Sigma_c \cup \Sigma_m \cup
\Sigma_s, \quad \Sigma_\bot^0 \subseteq \Sigma_\bot\,.\]
and for each $D$ over $\Sigma_m$ that is consistent
with $\mathcal{O}$, there exists $I$ agreeing with $D$ over $\Sigma_c$
and containing $D$ over $\Sigma_m$ such that $I\models \mathcal{O}$
and $I$ is empty over $\Sigma_\bot$. Replacing in $\mathcal{O}$ the
predicates from $\Sigma_\bot$ with $\bot$, we get the module
$\mathcal{O}'$.

\emph{$\leadsto$ Query emptiness with closed predicates}. 

NB: most often not unique (examples). With only $\Sigma_c, \Sigma_f,
\Sigma_\bot$ we can do a greedy local 
search algorithm. We start with $\Sigma_c=\Sigma_c^0$ and $\Sigma_\bot
= \Sigma_\bot^0$. Try to botomize predicates not in $\Sigma_f^0 \cup
\Sigma_c$ one by one. When impossible, close one additional predicate
(maybe starting from $\Sigma_f^0$?). Then, continue bottomizing, etc. 

\subsection{Ontology reduction}

Given an ontology $\mathcal{O}'$ eliminate open predicates that are not 
needed for consistency checks. (That is, we get the same models over
the smaller signature). How about: not needed for query answering over
$\Sigma_c \cup \Sigma_m \cup \Sigma_f^0$

\emph{$\leadsto$ Forgetting with closed predicates}. 


\subsection{Constraints extraction (compilation?)}

We need to make sure that the database is consistent. We will run
consistency checks each time a tuple is added or deleted. Would be
nice to make it as simple as possible.  Can we replace $\mathcal{O}'$
with a bunch of constraints over $\Sigma_c\cup \Sigma_m$. 
For which logics can we do it always? For which logics can we check if
it is doable, and do it if possible? For instance, for some logics one
can get an equivalent datalog program with rules of the forms $A(x) \lor \bar A
(x) \leftarrow$ and  $\bot \leftarrow A_1(x), \dots, A_n(x)$ and $\bot
\leftarrow A(x), r(x,y), A'(y)$. Can we get an equivalent datalog program
without intensional predicatese at all? If logics are Horn, instead of
disjunctive assertions you can get rules of the form $A(x) \leftarrow
A_1(x), \dots, A_n(x)$. It could be easier then. If no recursion,
immediate. 

\subsection{Query answering}
  
  Over the reduced module. For queries $Q_i$ it reduces to

  \emph{$\leadsto$ Consistency with closed predicates}

  because one can put the query in the ABox, and if there is a model where this is satisfied, then it is satisfied
  in each model. For other queries, use standard

  \emph{$\leadsto$ Query answering with closed predicates}.


\section{Reasoning modes}

There are two reasoning modes: finite and unrestricted. Which mode we
use depends on the modeling choices made when the ontology was
designed. So, each ontology should come with an indication of the
intended mode. When you choose to forget that not everybody had
parents, you should not use finite mode, because you introduce
additional inaccuracies.

If we choose the finite mode, all the tasks are performed in the finite. But if we choose
unrestricted mode, schema extraction reduces to QA in the mixed mode:
some relations are to be finite, some others can be infinite.  


\section{Proof of concept: $\mathcal{ALCOI}$}

Because of FMP and FC, the two (three) modes coincide.
\begin{description}
\item[Schema extraction] Known.
\item[Module extration] We just did it.
\item[Ontology reduction] Forgetting?
\item[Constraints extraction]
\item[Query answering]
\end{description}

\section{Proof of concept: \normalfont{\textsf{DL-Lite}}}

No FMP and FC, so the two modes diverge. Finite mode: all done? Not
sure... 

Unrestricted: 
\begin{description}
\item[Schema extraction] mixed QA done in the old draft. 
\item[Module extraction] TODO. 
\item[Ontology reduction] Forgetting?
\item[Constraints extraction]
\item[Query answering]
\end{description}


\section{Loose ends}

\begin{itemize}
\item
  Mixed QA for ALCIF doable by Ian Pratt-Hartmann.
\item
  In the definition of module extraction, once could allow $D$ to
  be an instance over $\Sigma_m \cup \Sigma_f$, while still keeping
  $\Sigma_f$ open. This would correspond to a setting where one
  populates open predicates as well. One could say they are a part of the
  database, but are not assumed closed. The original definition
  assumes that open predicates are only kept in the ontology and are
  static. 
\end{itemize}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:




==> equations.tex <==
\clearpage
  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:



